Does Configuration Encoding Matter in Learning Software Performance? An Empirical Study on Encoding Schemes

Learning and predicting the performance of a configurable software system helps to provide better quality assurance. One important engineering decision therein is how to encode the configuration into the model built. Despite the presence of different encoding schemes, there is still little understanding of which is better and under what circumstances, as the community often relies on some general beliefs that inform the decision in an ad-hoc manner. To bridge this gap, in this paper, we empirically compared the widely used encoding schemes for software performance learning, namely label, scaled label, and one-hot encoding. The study covers five systems, seven models, and three encoding schemes, leading to 105 cases of investigation. Our key findings reveal that: (1) conducting trial-and-error to find the best encoding scheme in a case by case manner can be rather expensive, requiring up to 400+ hours on some models and systems; (2) the one-hot encoding often leads to the most accurate results while the scaled label encoding is generally weak on accuracy over different models; (3) conversely, the scaled label encoding tends to result in the fastest training time across the models/systems while the one-hot encoding is the slowest; (4) for all models studied, label and scaled label encoding often lead to relatively less biased outcomes between accuracy and training time, but the paired model varies according to the system. We discuss the actionable suggestions derived from our findings, hoping to provide a better understanding of this topic for the community. To promote open science, the data and code of this work can be publicly accessed at https://github.com/ideas-labo/MSR2022-encoding-study.

==> Figures/exp.tex <==
% CS Table for RQ2
\begin{table*}[t!]
    % \caption{Scott-Knott rank on MHPerf~(with or without comments, which are highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{blue!10}{blue} and \setlength{\fboxsep}{1.5pt}\colorbox{red!10}{red}, respectively) against state-of-the-arts. The formats are the same as Table}
      \caption{Scott-Knott rankings and boxplot of RMSE of the 7 ML models with 3 encoding methods, for the 5 systems. 'OH', 'LAB' and 'SCA' stand for one-hot, label and scaled label encoding, respectively. A higher rank means the RMSE is lower and therefore the model with the encoding is better.}
    \label{tab:exp3}
  \begin{center}
    \begin{adjustbox}{max width = \textwidth}
     
\footnotesize
    \begin{tabular}{c@{}c@{}c}
        \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            % \cellcolor{blue!10}MHPerf & \cellcolor{blue!10}1 &\cellcolor{blue!10} 0.857 & \cellcolor{blue!10}0.025 & \cellcolor{blue!10} \quart{-5}{25}{85.7}{100}\\
NN\_SCA & 10 & 2944.45 & 0.39 & \quart{6.52}{0.39}{6.73}{100.00} \\
NN\_LAB & 10 & 2943.38 & 0.30 & \quart{6.57}{0.30}{6.73}{100.00} \\
NN\_OH & 10 & 2951.74 & 0.31 & \quart{6.64}{0.31}{6.75}{100.00} \\
KRR\_OH & 9 & 3014.68 & 0.19 & \quart{6.78}{0.19}{6.89}{100.00} \\
LR\_OH & 8 & 3020.36 & 0.21 & \quart{6.79}{0.21}{6.91}{100.00} \\
LR\_LAB & 8 & 3019.55 & 0.19 & \quart{6.80}{0.19}{6.91}{100.00} \\
RF\_SCA & 8 & 3019.63 & 0.20 & \quart{6.79}{0.20}{6.91}{100.00} \\
RF\_LAB & 8 & 3019.52 & 0.20 & \quart{6.79}{0.20}{6.91}{100.00} \\
KRR\_LAB & 8 & 3024.03 & 0.19 & \quart{6.81}{0.19}{6.92}{100.00} \\
LR\_SCA & 8 & 3026.49 & 0.19 & \quart{6.83}{0.19}{6.92}{100.00} \\
KRR\_SCA & 8 & 3028.21 & 0.19 & \quart{6.83}{0.19}{6.93}{100.00} \\
RF\_OH & 7 & 3060.11 & 0.20 & \quart{6.86}{0.20}{7.00}{100.00} \\
DT\_SCA & 6 & 3093.12 & 0.21 & \quart{7.00}{0.21}{7.07}{100.00} \\
DT\_LAB & 6 & 3097.61 & 0.22 & \quart{6.98}{0.22}{7.08}{100.00} \\
DT\_OH & 6 & 3095.11 & 0.25 & \quart{7.00}{0.25}{7.08}{100.00} \\
KNN\_SCA & 5 & 8968.09 & 1.54 & \quart{19.90}{1.54}{20.51}{100.00} \\
KNN\_OH & 4 & 15772.52 & 0.85 & \quart{35.78}{0.85}{36.07}{100.00} \\
KNN\_LAB & 3 & 22114.97 & 0.99 & \quart{49.96}{0.99}{50.57}{100.00} \\
SVR\_OH & 2 & 41917.30 & 5.73 & \quart{92.16}{5.73}{95.86}{100.00} \\
SVR\_SCA & 1 & 42228.88 & 5.85 & \quart{92.76}{5.85}{96.57}{100.00} \\
SVR\_LAB & 1 & 42229.54 & 5.86 & \quart{92.77}{5.86}{96.57}{100.00} \\

        \end{tabular} & 
        \begin{tabular}{|lcccl}
           \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            NN\_OH & 12 & 2497.07 & 0.10 & \quart{0.61}{0.10}{0.67}{100.00} \\
NN\_SCA & 11 & 2887.66 & 0.20 & \quart{0.72}{0.20}{0.78}{100.00} \\
NN\_LAB & 10 & 3019.11 & 0.34 & \quart{0.71}{0.34}{0.81}{100.00} \\
DT\_SCA & 9 & 15621.77 & 5.92 & \quart{2.61}{5.92}{4.19}{100.00} \\
DT\_LAB & 9 & 15621.69 & 5.92 & \quart{2.61}{5.92}{4.19}{100.00} \\
RF\_SCA & 8 & 25417.20 & 3.37 & \quart{5.50}{3.37}{6.82}{100.00} \\
RF\_LAB & 8 & 25457.00 & 3.18 & \quart{5.70}{3.18}{6.83}{100.00} \\
DT\_OH & 7 & 59610.67 & 9.35 & \quart{10.61}{9.35}{16.00}{100.00} \\
RF\_OH & 7 & 57173.71 & 5.31 & \quart{13.27}{5.31}{15.35}{100.00} \\
KNN\_LAB & 6 & 121668.37 & 3.96 & \quart{30.25}{3.96}{32.66}{100.00} \\
KNN\_SCA & 5 & 151716.91 & 3.54 & \quart{38.37}{3.54}{40.73}{100.00} \\
KNN\_OH & 4 & 168726.75 & 2.81 & \quart{43.77}{2.81}{45.30}{100.00} \\
KRR\_OH & 3 & 192199.55 & 3.73 & \quart{49.63}{3.73}{51.60}{100.00} \\
LR\_OH & 2 & 193658.25 & 3.88 & \quart{49.99}{3.88}{51.99}{100.00} \\
LR\_SCA & 2 & 194094.27 & 3.76 & \quart{50.36}{3.76}{52.11}{100.00} \\
LR\_LAB & 2 & 194648.94 & 3.79 & \quart{50.50}{3.79}{52.26}{100.00} \\
KRR\_SCA & 2 & 194588.83 & 3.84 & \quart{50.46}{3.84}{52.24}{100.00} \\
KRR\_LAB & 2 & 195128.40 & 3.88 & \quart{50.53}{3.88}{52.39}{100.00} \\
SVR\_LAB & 1 & 321782.26 & 6.84 & \quart{83.61}{6.84}{86.39}{100.00} \\
SVR\_OH & 1 & 321878.92 & 6.86 & \quart{83.64}{6.86}{86.42}{100.00} \\
SVR\_SCA & 1 & 321923.45 & 6.86 & \quart{83.65}{6.86}{86.43}{100.00} \\
        \end{tabular} &
                \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}
            \\
            \hline
            NN\_SCA & 12 & 398.39 & 8.37 & \quart{17.59}{8.37}{20.93}{100.00} \\
NN\_LAB & 12 & 398.39 & 8.37 & \quart{17.59}{8.37}{20.93}{100.00} \\
NN\_OH & 11 & 645.28 & 9.91 & \quart{27.93}{9.91}{33.90}{100.00} \\
RF\_LAB & 10 & 893.39 & 9.60 & \quart{42.73}{9.60}{46.93}{100.00} \\
RF\_SCA & 10 & 896.18 & 9.25 & \quart{42.81}{9.25}{47.08}{100.00} \\
RF\_OH & 9 & 947.02 & 11.43 & \quart{46.49}{11.43}{49.75}{100.00} \\
DT\_OH & 8 & 1104.22 & 12.32 & \quart{51.41}{12.32}{58.01}{100.00} \\
DT\_LAB & 7 & 1140.59 & 17.93 & \quart{53.16}{17.93}{59.92}{100.00} \\
DT\_SCA & 7 & 1140.63 & 17.93 & \quart{53.16}{17.93}{59.92}{100.00} \\
KNN\_OH & 6 & 1302.37 & 7.61 & \quart{63.67}{7.61}{68.42}{100.00} \\
KNN\_SCA & 5 & 1359.37 & 7.14 & \quart{68.06}{7.14}{71.41}{100.00} \\
KRR\_OH & 4 & 1378.64 & 8.30 & \quart{68.47}{8.30}{72.42}{100.00} \\
KRR\_SCA & 3 & 1410.46 & 9.14 & \quart{70.32}{9.14}{74.10}{100.00} \\
KRR\_LAB & 3 & 1411.00 & 9.15 & \quart{70.34}{9.15}{74.12}{100.00} \\
LR\_LAB & 3 & 1412.19 & 9.08 & \quart{70.45}{9.08}{74.19}{100.00} \\
LR\_SCA & 3 & 1411.56 & 9.14 & \quart{70.39}{9.14}{74.15}{100.00} \\
LR\_OH & 3 & 1411.28 & 10.07 & \quart{69.94}{10.07}{74.14}{100.00} \\
KNN\_LAB & 2 & 1502.74 & 10.07 & \quart{73.73}{10.07}{78.94}{100.00} \\
SVR\_OH & 1 & 1521.08 & 11.72 & \quart{75.65}{11.72}{79.91}{100.00} \\
SVR\_SCA & 1 & 1525.33 & 11.75 & \quart{75.84}{11.75}{80.13}{100.00} \\
SVR\_LAB & 1 & 1525.57 & 11.74 & \quart{75.85}{11.74}{80.14}{100.00} \\
        \end{tabular} \\
         \textbf{(a). \texttt{MongoDB}} & \textbf{(b). \texttt{Irzip}} & \textbf{(c). \texttt{Trimesh}}
        \\
        \\


        \begin{tabular}{|lcccl|}
            \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \cellcolor[gray]{1}\textbf{Med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
NN\_OH & 14 & 67.62 & 0.88 & \quart{3.18}{0.88}{3.38}{100.00} \\
NN\_LAB & 13 & 86.18 & 0.61 & \quart{4.05}{0.61}{4.31}{100.00} \\
NN\_SCA & 13 & 92.37 & 1.60 & \quart{3.97}{1.60}{4.62}{100.00} \\
RF\_OH & 12 & 164.02 & 3.99 & \quart{6.76}{3.99}{8.21}{100.00} \\
RF\_LAB & 12 & 159.83 & 4.00 & \quart{6.73}{4.00}{8.00}{100.00} \\
RF\_SCA & 12 & 158.61 & 4.00 & \quart{6.63}{4.00}{7.93}{100.00} \\
DT\_SCA & 11 & 179.07 & 3.46 & \quart{8.04}{3.46}{8.96}{100.00} \\
DT\_LAB & 11 & 181.96 & 3.40 & \quart{8.20}{3.40}{9.10}{100.00} \\
DT\_OH & 11 & 182.42 & 3.42 & \quart{8.23}{3.42}{9.13}{100.00} \\
KRR\_OH & 10 & 369.58 & 0.95 & \quart{18.17}{0.95}{18.49}{100.00} \\
KNN\_SCA & 10 & 363.34 & 2.40 & \quart{17.65}{2.40}{18.18}{100.00} \\
KNN\_OH & 9 & 438.83 & 1.24 & \quart{21.43}{1.24}{21.95}{100.00} \\
KNN\_LAB & 8 & 1008.23 & 1.43 & \quart{49.62}{1.43}{50.44}{100.00} \\
KRR\_LAB & 7 & 1113.89 & 1.61 & \quart{54.82}{1.61}{55.72}{100.00} \\
SVR\_OH & 6 & 1210.97 & 1.25 & \quart{59.93}{1.25}{60.58}{100.00} \\
KRR\_SCA & 5 & 1306.24 & 1.56 & \quart{64.59}{1.56}{65.34}{100.00} \\
SVR\_LAB & 4 & 1495.85 & 1.82 & \quart{74.05}{1.82}{74.83}{100.00} \\
SVR\_SCA & 3 & 1507.12 & 1.92 & \quart{74.76}{1.92}{75.39}{100.00} \\
LR\_SCA & 2 & 4562.24 & 1.97 & \quart{90.10}{1.97}{92.82}{100.00} \\
LR\_LAB & 2 & 4483.84 & 2.12 & \quart{90.72}{2.12}{92.45}{100.00} \\
LR\_OH & 1 & 7814.81 & 99 & \quart{90.70}{9}{99.11}{100.00} \\


        \end{tabular} &
        \begin{tabular}{lcccl}
              \cellcolor[gray]{1}\textbf{Classifier} & \cellcolor[gray]{1}\textbf{Rank} &     \hphantom{\cellcolor[gray]{1}\textbf{Med}} & \hphantom{\cellcolor[gray]{1}\textbf{IQR}} & \hphantom{\cellcolor[gray]{1}}\\
            \hline
RF\_LAB & 19 & 581.18 & 6.07 & \quart{27.64}{6.07}{29.07}{100.00} \\
NN\_OH & 19 & 446.49 & 7.94 & \quart{19.60}{7.94}{22.34}{100.00} \\
NN\_LAB & 18 & 481.45 & 6.97 & \quart{20.77}{6.97}{24.08}{100.00} \\
NN\_SCA & 17 & 671.84 & 5.32 & \quart{31.75}{5.32}{33.61}{100.00} \\
RF\_OH & 17 & 665.35 & 6.60 & \quart{30.65}{6.60}{33.28}{100.00} \\
KNN\_OH & 16 & 1021.07 & 4.49 & \quart{48.97}{4.49}{51.08}{100.00} \\
RF\_SCA & 15 & 735.36 & 4.61 & \quart{35.10}{4.61}{36.79}{100.00} \\
DT\_LAB & 14 & 739.20 & 6.96 & \quart{34.49}{6.96}{36.98}{100.00} \\
KRR\_OH & 13 & 910.47 & 4.64 & \quart{43.52}{4.64}{45.55}{100.00} \\
DT\_OH & 12 & 803.96 & 8.26 & \quart{36.70}{8.26}{40.22}{100.00} \\
DT\_SCA & 11 & 950.32 & 6.04 & \quart{45.36}{6.04}{47.54}{100.00} \\
LR\_LAB & 10 & 1046.27 & 3.38 & \quart{50.07}{3.38}{52.34}{100.00} \\
KNN\_SCA & 9 & 939.14 & 3.79 & \quart{45.49}{3.79}{46.98}{100.00} \\
LR\_SCA & 8 & 1084.04 & 3.01 & \quart{53.02}{3.01}{54.23}{100.00} \\
KRR\_LAB & 7 & 1110.85 & 3.61 & \quart{53.77}{3.61}{55.57}{100.00} \\
KRR\_SCA & 6 & 1183.43 & 3.39 & \quart{57.17}{3.39}{59.20}{100.00} \\
KNN\_LAB & 5 & 1455.11 & 4.34 & \quart{70.68}{4.34}{72.79}{100.00} \\
SVR\_LAB & 4 & 1487.67 & 4.93 & \quart{72.13}{4.93}{74.42}{100.00} \\
SVR\_OH & 3 & 1566.62 & 5.47 & \quart{76.28}{5.47}{78.37}{100.00} \\
SVR\_SCA & 2 & 1714.36 & 5.89 & \quart{83.50}{5.89}{85.76}{100.00} \\
LR\_OH & 1 & 9999.99 & 17.91 & \quart{90}{17}{99}{100.00} \\

        \end{tabular}\\
      \textbf{(d). \texttt{ExaStencils}}  & \textbf{(e). \texttt{X264-DB}}\\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}

==> tables/key-options.tex <==
\begin{table}[!t]
\caption{The key configuration options identified.}
\label{tb:keyopt}
\centering
%\setlength{\tabcolsep}{1.1mm}
%\scriptsize
\footnotesize
%\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ccc|cc}
\toprule
    \textbf{System}&
    $\lvert \mathbfcal{P} \rvert$&
    \textbf{Key Option(s)}&
    $\lvert \mathbfcal{P} \rvert$&
    \textbf{Key Option(s)}\\
    \midrule
    






\textsc{Storm/WC-Azure}&
P1&
\texttt{spout\_wait}&
P2&
\texttt{spout\_wait}\\


\rowcolor{blue!10}\textsc{Storm/WC-ON-3}&
P1&
\texttt{spout\_wait}&
P2&
\texttt{spout\_wait}\\

\textsc{Storm/2WC-EC2}&
P1&
\texttt{max\_spout}, \texttt{spliter}&
P2&
\texttt{max\_spout}\\


\rowcolor{blue!10}\textsc{Storm/WC-RS-EC2}&
P1&
\texttt{max\_spout}&
P2&
\texttt{max\_spout}\\


\textsc{Storm/WC-ON-5}&
P1&
\texttt{spout}&
P2&
\texttt{count}\\


\rowcolor{blue!10}\textsc{Sort-256}&
P1&
\texttt{sort\_a}, \texttt{sort\_b}&
P2&
\texttt{sort\_a}\\


\textsc{non-CM-log}&
P1&
\texttt{multiplier}&
P2&
\texttt{multiplier}\\






    
     
   \bottomrule
   
   %\quart{of 0}{16}{10}{20}
    %\rowcolor{blue!10}\textbf{5} & \textbf{D1} & \textbf{0.80} & \textbf{0.14} & \quart{71}{14}{80}{100}\\
\end{tabular}
\centering
 \begin{tablenotes}
    \footnotesize
    \item $\lvert \mathbfcal{P} \rvert$ denotes the performance attribute.
    \end{tablenotes}
\end{table}

==> tables/rq1/rq1.tex <==
\begin{table*}[!t]
\caption{The median difference (IQR) on RMSE over 50 runs; \colorbox{blue!10}{blue cell} denotes the label encoding wins while \colorbox{red!10}{red cell} denotes the label encoding loses; white cell means a tie. N, S, M, and L denotes negligible, small, medium, and large effect size, respectively. $^\dagger$ means the comparison has a $p<0.05$. Statistically significant comparison with non-trivial effect size is shown in bold.}
\label{tb:rq1}
\centering
\setlength{\tabcolsep}{0.5mm}
%\scriptsize
\footnotesize
%\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ccll|ll|ll|ll|ll|ll}
\toprule
    &&\multicolumn{2}{c}{\textbf{RF}} & \multicolumn{2}{c}{\textbf{$k$NN}} & \multicolumn{2}{c}{\textbf{SVR}} & \multicolumn{2}{c}{\textbf{DT}} & \multicolumn{2}{c}{\textbf{LR}} & \multicolumn{2}{c}{\textbf{KRR}}  \\
    \midrule
    
%    wc-c1-3d (SS-A)
%    wc-3c-3d (SS-C)
%    wc+wc-c4-3d (SS-D)
%    wc+rs-c4-3d (SS-F)
%    wc-5d-c5 (SS-I)
%    sort-256 (SS-B)
%    noc-CM-log (SS-H)

    
\multirow{2}{*}{\textsc{Storm/WC-Azure}}&P1&   

\cellcolor{blue!10}$-$0.90 (1.50) & \cellcolor{blue!10}N$^\dagger$
    &  \cellcolor{blue!10}{41.83 (48.18)}&\cellcolor{blue!10}{N$^\dagger$}
    &  both timeout&
    &  \cellcolor{red!10}$-$1.33 (2.34)&\cellcolor{red!10}N$^\dagger$
    &  \textbf{\cellcolor{red!10}$-$124.96 (65.42)}&\textbf{\cellcolor{red!10}S$^\dagger$}
    &  \cellcolor{blue!10}$-$73.50 (65.83) & \cellcolor{blue!10}N$^\dagger$\\
&P2&   
\cellcolor{red!10}{$-$0.94 (150.76)} & \cellcolor{red!10}{N}
    &  \cellcolor{blue!10}{9.80 (439.25)} & \cellcolor{blue!10}{N}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{blue!10}{9.92 (353.24)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{347.84 (220.10)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$739.91 (259.21)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
\hline

\multirow{2}{*}{\textsc{Storm/WC-ON-3}}
&P1&
\textbf{\cellcolor{blue!10}{172.44 (180.15)}}&\textbf{\cellcolor{blue!10}{L$^\dagger$}}
    & \cellcolor{blue!10}{449.19 (374.46)}&\cellcolor{blue!10}{N$^\dagger$}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{blue!10}{83.24 (178.90)}&\cellcolor{blue!10}{N$^\dagger$}
    &  \textbf{\cellcolor{red!10}{$-$1368.73 (614.68)}} & \textbf{\cellcolor{red!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1003.54 (720.35)}} & \textbf{\cellcolor{red!10}{S$^\dagger$}}\\
&P2&
\textbf{\cellcolor{blue!10}{1129.18 (519.65)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1283.71 (512.30)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{1438.48 (961.74)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{635.07 (307.12)}}&\textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1407.99 (354.30)}}&\textbf{\cellcolor{red!10}{L$^\dagger$}}\\
\hline
    
\multirow{2}{*}{\textsc{Storm/2WC-EC2}}
&P1&   
\textbf{\cellcolor{blue!10}{2870.99 (4862.44)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \cellcolor{blue!10}{1726.53 (3177.50)} & \cellcolor{blue!10}{N$^\dagger$}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{2037.28 (6914.90)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{7896.56 (10418.86)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \cellcolor{blue!10}{1009.15 (2757.00)} & \cellcolor{blue!10}{N$^\dagger$}\\
&P2&   
\textbf{\cellcolor{blue!10}{409.65 (1985.19)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{2363.43 (1986.66)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{blue!10}{235.80 (2662.56)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{4769.91 (7236.36)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{5990.96 (3483.08)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
\hline

\multirow{2}{*}{\textsc{Storm/WC-RS-EC2}}
&P1&   
\textbf{\cellcolor{blue!10}{1481.49 (6532.88)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{2529.33 (3890.78)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \cellcolor{blue!10}{113.87 (269.64)} & \cellcolor{blue!10}{N$^\dagger$}
    &  \textbf{\cellcolor{blue!10}{2158.02 (9754.71)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{9764.45 (15211.68)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1366.91 (4113.91)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}\\
&P2&   
\cellcolor{blue!10}{417.70 (1793.86)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{1965.56 (2704.00)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$6668.69 (10334.43)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}
    &  \cellcolor{blue!10}{480.83 (2436.13)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{3463.33 (8614.26)}} & \textbf{\cellcolor{blue!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{6087.9 (3206.82)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
\hline
    
\multirow{2}{*}{\textsc{STROM/WC-ON-5}}
&P1&   
\textbf{\cellcolor{blue!10}{2.54 (4.25)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{7.19 (5.11)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  both timeout&
    &  \cellcolor{blue!10}{0.02 (6.20)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{2.59 (4.45)}} & \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$10.35 (6.40)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
&P2&   
\cellcolor{blue!10}{4.60 (258.34)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{blue!10}{441.00 (164.80)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{682.53 (363.20)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$117.27 (186.78)}} & \textbf{\cellcolor{red!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1277.94 (342.23)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$2163.45 (791.86)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
\hline

\multirow{2}{*}{\textsc{Sort-256}}
&P1&   
\textbf{\cellcolor{blue!10}{0.88 (0.37)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.92 (0.35)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{0.94 (0.60)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.54 (0.38)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1.88 (1.02)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
&P2&   
\textbf{\cellcolor{blue!10}{0.68 (0.25)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.84 (0.44)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{0.76 (0.38)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.62 (0.44)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{1.99 (1.02)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}\\
\hline
    
\multirow{2}{*}{\textsc{noc-CM-log}}
&P1&   
\textbf{\cellcolor{blue!10}{0.17 (0.18)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \textbf{\cellcolor{blue!10}{0.49 (0.17)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \textbf{\cellcolor{blue!10}{0.09 (0.17)}}& \textbf{\cellcolor{blue!10}{S$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$0.06 (0.15)}} & \textbf{\cellcolor{red!10}{M$^\dagger$}}
    &  \textbf{\cellcolor{red!10}{$-$1.94 (0.47)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\
&P2&   \cellcolor{white!10}{0.00 (0.02)} & \cellcolor{white!10}{N$^\dagger$}
    &  \textbf{\cellcolor{blue!10}{0.04 (0.02)}} & \textbf{\cellcolor{blue!10}{L$^\dagger$}}
    &  \cellcolor{red!10}label timeout&\cellcolor{red!10}
    &  \cellcolor{white!10}{0.00 (0.04)} & \cellcolor{white!10}{N}
    &  \cellcolor{blue!10}{0.01 (0.04)} & \cellcolor{blue!10}{N}
    &  \textbf{\cellcolor{red!10}{$-$1.42 (0.27)}} & \textbf{\cellcolor{red!10}{L$^\dagger$}}\\



    
     
   \bottomrule
   
   %\quart{of 0}{16}{10}{20}
    %\rowcolor{blue!10}\textbf{5} & \textbf{D1} & \textbf{0.80} & \textbf{0.14} & \quart{71}{14}{80}{100}\\
\end{tabular}
%\end{adjustbox}
\end{table*}


==> tables/rq2/rq2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{The Scott-Knott test scores of the RMSE of the five subject systems; Each line represents the relative scoreings of the RMSE over 50 runs of each performance model with each encoding method. A higher scire means a lower RMSE, which means the results are better. If two results are of the same score, they have insignificant difference.}
\label{tb:rq2-acc}
\centering
\setlength{\tabcolsep}{0.9mm}
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc|ccc|ccc@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}DT} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KNN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KRR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}LR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}NN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}RF} &
  \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}SVR} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA \\
\rowcolor[HTML]{EFEFEF} 
MongoDB &
  6 &
  6 &
  6 &
  4 &
  3 &
  5 &
  9 &
  8 &
  8 &
  8 &
  8 &
  8 &
  10 &
  10 &
  10 &
  7 &
  8 &
  8 &
  2 &
  1 &
  1 \\
\rowcolor[HTML]{C0C0C0} 
Irzip &
  7 &
  9 &
  9 &
  4 &
  6 &
  5 &
  3 &
  2 &
  2 &
  2 &
  2 &
  2 &
  12 &
  10 &
  11 &
  7 &
  8 &
  8 &
  1 &
  1 &
  1 \\
\rowcolor[HTML]{EFEFEF} 
Trimesh &
  8 &
  7 &
  7 &
  6 &
  2 &
  5 &
  4 &
  3 &
  3 &
  3 &
  3 &
  3 &
  11 &
  12 &
  12 &
  9 &
  10 &
  10 &
  1 &
  1 &
  1 \\
\rowcolor[HTML]{C0C0C0} 
ExaStencils &
  11 &
  11 &
  11 &
  9 &
  8 &
  10 &
  10 &
  7 &
  5 &
  1 &
  2 &
  2 &
  14 &
  13 &
  13 &
  12 &
  12 &
  12 &
  6 &
  4 &
  3 \\
\rowcolor[HTML]{EFEFEF} 
X264-DB &
  14 &
  15 &
  11 &
  10 &
  5 &
  12 &
  13 &
  7 &
  6 &
  1 &
  9 &
  8 &
  19 &
  19 &
  17 &
  17 &
  18 &
  16 &
  3 &
  4 &
  2 \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/rq3/pareto.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{The pareto-optimal points considering the the Scott-Knott rankings of both RMSE and training time. The \colorbox{green!40}{green cells} represent the pareto-optimal cases, i.e., no other case for the same system is better than them in both accuracy and time.}
\label{tb:rq3-pareto}
\centering
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}DT} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KNN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KRR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}LR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}NN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}RF} &
  \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}SVR} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA \\
\rowcolor[HTML]{EFEFEF} 
MongoDB &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
   &
   \\
   \hline
\rowcolor[HTML]{C0C0C0} 
Irzip &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
   &
   \\
\rowcolor[HTML]{EFEFEF} 
   \hline
Trimesh &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   \\
\rowcolor[HTML]{C0C0C0} 
   \hline
ExaStencils &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   \\
\rowcolor[HTML]{EFEFEF} 
   \hline
X264-DB &
   &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
  \cellcolor[HTML]{9AFF99} &
   &
  \cellcolor[HTML]{9AFF99} &
   &
   &
   &
   \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/rq3/rq3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\caption{The Scott-Knott rank test results of the training time of the five subject systems; Each line represents the relative rankings of the training time over 50 runs of each performance model with each encoding method. A higher ranking means less training time, which means the results are better. If two results are of the same rank, they have insignificant difference.}
\label{tb:rq3-time}
\centering
\setlength{\tabcolsep}{0.9mm}
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc|ccc|ccc@{}}
\toprule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}DT} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KNN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}KRR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}LR} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}NN} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}RF} &
  \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}SVR} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}} & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA & OH & LAB & SCA \\
\rowcolor[HTML]{EFEFEF} 
MongoDB                                      & 13 & 17  & 16  & 14 & 15  & 12  & 6  & 2   & 8   & 18 & 19  & 19  & 10 & 7   & 11  & 1  & 9   & 4   & 3  & 5   & 1   \\
\rowcolor[HTML]{C0C0C0} 
Irzip                                        & 12 & 14  & 15  & 13 & 17  & 16  & 5  & 11  & 10  & 18 & 19  & 20  & 1  & 2   & 3   & 1  & 8   & 9   & 4  & 7   & 6   \\
\rowcolor[HTML]{EFEFEF} 
Trimesh                                      & 13 & 15  & 16  & 14 & 18  & 17  & 10 & 12  & 11  & 19 & 20  & 20  & 2  & 4   & 3   & 1  & 8   & 9   & 5  & 6   & 7   \\
\rowcolor[HTML]{C0C0C0} 
ExaStencils                                  & 12 & 14  & 15  & 13 & 17  & 16  & 10 & 4   & 11  & 18 & 19  & 20  & 5  & 2   & 3   & 1  & 9   & 8   & 5  & 6   & 7   \\
\rowcolor[HTML]{EFEFEF} 
X264-DB                                      & 11 & 17  & 15  & 12 & 16  & 14  & 7  & 10  & 6   & 13 & 19  & 18  & 3  & 5   & 8   & 2  & 4   & 3   & 1  & 5   & 9   \\ \bottomrule

\end{tabular}
\end{table*}
